ILID: Native Script Language Identification for Indian Languages

The language identification task is a crucial fundamental step in NLP. Often it serves as a pre-processing step for widely used NLP applications such as multilingual machine translation, information retrieval, question and answering, and text summarization. The core challenge of language identification lies in distinguishing languages in noisy, short, and code-mixed environments. This becomes even harder in case of diverse Indian languages that exhibit lexical and phonetic similarities, but have distinct differences. Many Indian languages share the same script, making the task even more challenging. Taking all these challenges into account, we develop and release a dataset of 250K sentences consisting of 23 languages including English and all 22 official Indian languages labeled with their language identifiers, where data in most languages are newly created. We also develop and release baseline models using state-of-the-art approaches in machine learning and fine-tuning pre-trained transformer models. Our models outperforms the state-of-the-art pre-trained transformer models for the language identification task. The dataset and the codes are available at https://yashingle-ai.github.io/ILID/ and in Huggingface open source libraries.

==> Dataset_Creation.tex <==
\section{ILID Dataset Creation}
\label{sec:dataset}
Indian Language IDentification (ILID) dataset is created using two approaches. We attempt to include English and all 22 official Indian languages \footnote{\url{https://en.wikipedia.org/wiki/Eighth_Schedule_to_the_Constitution_of_India}} widely used in India. The first approach utilizes web scraping for the languages in which the digital presence is significant (details are given in the Appendix). For each of these languages, we collect 10,000 different sentences from diverse sources such as government websites, newspapers, books, and other public materials ensuring varying degrees of linguistic complexity. The second approach samples sentences from an existing massive monolingual and parallel corpora for Indian languages \cite{mujadia2024bhashaversetranslationecosystem}.

To ensure quality and consistency, the dataset undergoes several noise removal steps. The first step involves the elimination of duplicate, very short, and ungrammatical sentences. The next step employs an existing FastText \cite{joulin2016bagtricksefficienttext,joulin2016fasttextzipcompressingtextclassification} based language identification model to remove sentences where the probability of detecting the language of the text is very low (we fix a threshold of 0.7 for this filtering process). This happens in code-mixed texts as many Indians are multilingual \footnote{\url{https://en.wikipedia.org/wiki/List_of_languages_by_number_of_native_speakers_in_India}} and often use more than one language while writing.

The first approach is described in details.
\subsection{Web Scraping}
To build a strong language identification system for Indian languages, we carefully built a personalized set of 10,000 text samples for each language, covering 22 Indian languages: Hindi, Bengali, Tamil, Telugu, Marathi, Gujarati, Kannada, Malayalam, Odia, Punjabi, Assamese, English, Urdu, Dogri, Bodo, Goan Konkani, Kashmiri, Manipuri (Meitei), Santali, Sindhi, Maithili, Nepali.

Text data was collected from a variety of publicly available and diverse sources, including:
Wikipedia dumps in respective languages for formal and structured text.
News websites and blogs for professional and personal updates. All efforts were made to ensure the samples were multilingual in length, script (i.e., Devanagari, Bengali, Tamil, etc.), domain, and style, reflecting the multilingual nature of India.

For a target website $W$, we define the scraping process as:

\begin{equation}
    S(W) = \bigcup_{p \in P_W} \phi(p)
\end{equation}

where $P_W$ is the set of target pages and $\phi$ is the extraction function that parses HTML content while preserving structural information. We implement adaptive throttling using:

\begin{equation}
    \Delta_t = \frac{1}{|W|} \sum_{i=1}^{|W|} \frac{\text{size}(w_i)}{\text{bandwidth}}
\end{equation}

\subsection{Data Cleaning Pipeline}
In the data cleaning process we mainly work on removing extra spaces, extra special symbols, unicode normalization, breaking the paragraph into meaningful sentences, and after that we apply various tokenisation methods. For sentence tokenization, we utilized the corresponding Devanagari script. We have explained all our processes in detail.
Our cleaning process transforms raw text $T$ to cleaned text $T'$ through:

\begin{equation}
    T' = \psi_n(\psi_s(T))
\end{equation}

where $\psi_s$ handles special characters and $\psi_n$ performs normalization.

==> language_wise_table_word_feature_report.tex <==

\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{0.64\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Language} & \textbf{LR} & \textbf{DT} & \textbf{RF} & \textbf{SVM} & \textbf{SGD} & \textbf{k-NN} & \textbf{NB} & \textbf{AdaBoost} \\ \hline
Assamese (asm)    & 0.99 & 0.96 & 0.98 & \textbf{0.99} & 0.98 & 0.91 & 0.97 & 0.78 \\ \hline
Bengali (ben)     & \textbf{1.00} & 0.98 & 0.99 & \textbf{1.00} & 0.99 & 0.93 & 0.99 & 0.93 \\ \hline
Bodo (brx)        & 0.95 & 0.90 & \textbf{0.96} & \textbf{0.96} & 0.95 & 0.89 & 0.96 & 0.69 \\ \hline
Dogri (doi)       & \textbf{0.91} & 0.82 & \textbf{0.91} & 0.90 & 0.88 & 0.71 & \textbf{0.91} & 0.21 \\ \hline
English (eng)     & \textbf{1.00} & \textbf{1.00} & 0.99 & \textbf{1.00} & 0.99 & \textbf{1.00} & 0.99 & 0.96 \\ \hline
Konkani (gom)     & \textbf{0.97} & 0.86 & 0.94 & \textbf{0.97} & 0.92 & 0.81 & 0.95 & 0.31 \\ \hline
Gujarati (guj)    & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.97 \\ \hline
Hindi (hin)       & 0.99 & 0.93 & 0.98 & \textbf{0.99} & 0.97 & 0.84 & 0.94 & 0.74 \\ \hline
Kannada (kan)     & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.96 \\ \hline
Kashmiri (kas)    & 0.98 & 0.93 & 0.97 & 0.98 & 0.94 & \textbf{0.98} & \textbf{0.98} & 0.74 \\ \hline
Maithili (mai)    & \textbf{0.85} & 0.78 & 0.84 & \textbf{0.85} & 0.81 & 0.67 & 0.82 & 0.26 \\ \hline
Malayalam (mal)   & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.97 \\ \hline
Marathi (mar)     & 0.97 & 0.85 & 0.95 & \textbf{0.98} & 0.92 & 0.79 & 0.94 & 0.50 \\ \hline
Manipuri (mni)    & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.99 & \textbf{1.00} & 0.89 \\ \hline
Nepali (npi)      & 0.90 & 0.84 & 0.90 & 0.90 & 0.86 & 0.76 & \textbf{0.89} & 0.28 \\ \hline
Odia (ory)        & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.90 \\ \hline
Punjabi (pan)     & \textbf{1.00} & 0.99 & 0.99 & \textbf{1.00} & 0.99 & 0.99 & \textbf{1.00} & 0.91 \\ \hline
Santali (sat)     & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.94 \\ \hline
Sindhi (snd)      & 0.94 & 0.87 & 0.93 & 0.93 & 0.90 & 0.80 & \textbf{0.92} & 0.23 \\ \hline
Tamil (tam)       & \textbf{1.00} & 0.99 & \textbf{1.00} & \textbf{1.00} & 0.99 & \textbf{1.00} & \textbf{1.00} & 0.96 \\ \hline
Telugu (tel)      & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.92 \\ \hline
Urdu (urd)        & 0.98 & 0.92 & 0.97 & \textbf{0.99} & 0.96 & 0.98 & \textbf{0.98} & 0.75 \\ \hline
\hline
\textbf{Macro Avg} & 0.97 & 0.94 & 0.97 & 0.97 & 0.96 & 0.91 & 0.96 & 0.72 \\ \hline
\end{tabular}
}


\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{0.64\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Language} & \textbf{LR} & \textbf{DT} & \textbf{RF} & \textbf{SVM} & \textbf{SGD} & \textbf{k-NN} & \textbf{NB} & \textbf{ADABoost} \\ \hline
Assamese (asm)    & 0.99 & 0.97 & 0.99 & 0.99 & 0.98 & 0.91 & 0.98 & 0.77 \\ \hline
Bengali (ben)     & 1.00 & 0.99 & 0.99 & 1.00 & 0.99 & 0.93 & 0.99 & 0.92 \\ \hline
Bodo (brx)        & 0.96 & 0.92 & 0.96 & 0.97 & 0.94 & 0.90 & 0.96 & 0.68 \\ \hline
Dogri (doi)       & 0.90 & 0.82 & 0.89 & 0.90 & 0.88 & 0.71 & 0.90 & 0.19 \\ \hline
English (eng)     & 1.00 & 0.99 & 1.00 & 1.00 & 1.00 & 1.00 & 0.99 & 0.95 \\ \hline
Konkani (gom)     & 0.97 & 0.85 & 0.95 & 0.97 & 0.93 & 0.80 & 0.96 & 0.29 \\ \hline
Gujarati (guj)    & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.97 \\ \hline
Hindi (hin)       & 0.99 & 0.93 & 0.99 & 0.99 & 0.98 & 0.83 & 0.94 & 0.79 \\ \hline
Kannada (kan)     & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.96 \\ \hline
Kashmiri (kas)    & 0.99 & 0.95 & 0.97 & 0.99 & 0.94 & 0.97 & 0.98 & 0.75 \\ \hline
Maithili (mai)    & 0.87 & 0.78 & 0.84 & 0.86 & 0.84 & 0.67 & 0.84 & 0.26 \\ \hline
Malayalam (mal)   & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.96 \\ \hline
Marathi (mar)     & 0.98 & 0.84 & 0.96 & 0.98 & 0.93 & 0.76 & 0.94 & 0.52 \\ \hline
Manipuri (mni)    & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.90 \\ \hline
Nepali (npi)      & 0.92 & 0.84 & 0.90 & 0.91 & 0.86 & 0.76 & 0.89 & 0.28 \\ \hline
Odia (ory)        & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.90 \\ \hline
Punjabi (pan)     & 1.00 & 0.99 & 1.00 & 1.00 & 0.99 & 0.99 & 0.99 & 0.91 \\ \hline
Santali (sat)     & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.95 \\ \hline
Sindhi (snd)      & 0.94 & 0.86 & 0.92 & 0.93 & 0.90 & 0.80 & 0.94 & 0.24 \\ \hline
Tamil (tam)       & 1.00 & 0.99 & 1.00 & 1.00 & 0.99 & 0.99 & 0.99 & 0.95 \\ \hline
Telugu (tel)      & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.91 \\ \hline
Urdu (urd)        & 0.99 & 0.94 & 0.96 & 0.99 & 0.96 & 0.97 & 0.98 & 0.76 \\ \hline
\end{tabular}
}
\caption{Test dataset report: word + char  analyzer F1-score comparison across 22 Indian languages for different classifiers.}
\label{tab:f1_scores}
\end{table}

